A Rowhammer attack on Fil-C's software capabilities

Fil-C retrofits spatial and temporal memory safety onto C/C++ using software capabilities (bounds that are checked at every pointer dereference). Fil-C's guarantee rests on an unstated hardware assumption: that DRAM preserves the capabilities. We show that Rowhammer breaks it. In Fil-C 0.679 a part of each heap pointer's capability lives in a 16-byte header stored inline in ordinary DRAM immediately before the object pointed to, with no mechanism to prevent capabilities from corruption. A single 0 &rarr; 1 bit flip in the capability's upper-bound expands the pointer's permitted range by 2<sup>k</sup> bytes and is invisible to the runtime, raising no panic or signal. We demonstrate this by using Fil-C to <i>convert</i> existing Rowhammer attacks into concrete attacks against a heterogeneous collection of victim software. To aid reproducibility (not everybody has DRAM vulnerable to Rowhammer) we split our demonstration into two paths. First, along a <i>deterministic path</i>, we isolate Fil-C as a novel attack vector using a deterministic, Rowhammer-like fault-injection model. Across four case studies, this model corrupts the upper-bound word of a pointer, permitting previously out-of-bounds reads and writes. We use this to achieve a bounded read/write window, secret disclosure, privilege escalation by flipping an adjacent <code>is_admin</code> field, and the leakage of a tenant API key in a multi-tenant credential service backed by SQLite (compiled under Fil-C). Second, along a <i>physical end-to-end path</i>, we demonstrate all four attacks on real hardware equipped with DDR3 memory, and with Target Row Refresh (TRR) equipped DDR4, proving the exploits are physically realisable. The latter attack shows that the TRR defence does not close the Fil-C delivery channel. We close with a discussion of Fil-C-specific mitigations.

==> figures/dram_rows.tex <==
\begin{figure}[t]
\centering
%% Three physical rows: aggressor A (top), victim (middle), aggressor B (bot)
%% Row coords: row A y=1.44..2.09, row V y=0.72..1.37, row B y=0.00..0.65
\begin{tikzpicture}[font=\scriptsize]
  \node[drow,fill=rowAcol,minimum width=3.20cm] (rA) at (1.60,1.800)
        {Aggressor $r_A$ (attacker pool)};
  \node[drow,fill=rowVcol,minimum width=3.20cm] (rV) at (1.60,0.850)
        {Victim $r_V$ (\InvisiCap{} slab)};
  \node[drow,fill=rowAcol,minimum width=3.20cm] (rB) at (1.60,-0.100)
        {Aggressor $r_B$ (attacker pool)};
  %% Disturbance arrows
  \draw[->,very thick,red!55] (1.60,1.50) -- (1.60,1.15);
  \draw[->,very thick,red!55] (1.60,0.20) -- (1.60,0.55);
  %% Bit-flip marker in victim row
  \draw[draw=orange!75,fill=orange!22,line width=0.5pt]
        (2.70,0.67) rectangle (3.10,1.02);
  \node[font=\tiny\bfseries,text=orange!85] at (2.90,0.92) {0$\!\to\!$1};
  \node[font=\tiny,text=orange!75]          at (2.90,0.77) {bit $k$};
  %% Equation callout
  \node[draw=gray!45,fill=gray!7,rounded corners=2pt,font=\tiny,
        text width=3.1cm, align=center] at (1.60,-1)
      {$u'=u+2^k$\quad (Eq.~\ref{eq:expansion})\\
       \FilC{} check passes for all\\
       $\mathtt{access}\in[u,\;u+2^k)$};
\end{tikzpicture}
\caption{Double-sided Rowhammer targeting the \InvisiCap{} slab row.
Hammering $r_A$ and $r_B$ from the attacker's hugepage pool disturbs
$r_V$, flipping bit~$k$ of \texttt{upper\_bound} and expanding the
permitted access range by $2^k$\,bytes.}
\label{fig:dram_rows}
\end{figure}


==> figures/grooming.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[x=0.62cm, y=0.9cm, font=\scriptsize]
  %% (top) physical frames donated to the allocator; two are known-flippy
  \node[anchor=east,font=\tiny] at (-0.3,2) {Donated frames};
  \foreach \i in {0,1,3,4,6,7}{
    \node[slt,fill=slotempty] at (\i,2) {};
  }
  \node[slt,fill=orange!22,draw=orange!70,line width=0.6pt,text=orange!85]
       at (2,2) {$\star$};
  \node[slt,fill=orange!22,draw=orange!70,line width=0.6pt,text=orange!85]
       at (5,2) {$\star$};
  \node[font=\tiny,text=orange!80,anchor=west] at (7.6,2) {flippy};

  %% (bottom) victim sprays same-size-class objects; cap words fill frames
  \node[anchor=east,font=\tiny] at (-0.3,0.55) {Sprayed cap words};
  \foreach \i in {0,1,2,3,4,6,7}{
    \node[slt,fill=slotfull] at (\i,0.55) {\tiny cap};
  }
  \node[slt,fill=slottgt,draw=red!55,line width=0.7pt] at (5,0.55)
       {\tiny\bfseries cap};

  %% each sprayed object occupies the frame above it
  \foreach \i in {0,1,2,3,4,6,7}{ \draw[arr,gray!45] (\i,0.79) -- (\i,1.77); }
  \draw[arr,red!55] (5,0.79) -- (5,1.77);

  %% hammer the frame the winning cap word landed on
  \draw[->,red!60,thick] (5,2.62) -- (5,2.25)
        node[above,font=\tiny,text=red!65] at (5,2.5) {hammer};
\end{tikzpicture}
\caption{Flip Feng Shui grooming for the physical end-to-end.  The attacker
templates known-flippy physical frames and donates (frees) them to the
allocator; the victim sprays same-size-class objects until an \InvisiCap{}
upper-bound word lands on a donated flippy frame (highlighted).  Re-hammering
that frame flips bit~$k$ of the \emph{live} capability.  A two-phase spray
(scout, then main) first pins the memory zone the victim's allocator is
currently drawing from, so donations land in the right zone.}
\label{fig:grooming}
\end{figure}


==> figures/invisicaps.tex <==

\usetikzlibrary{decorations.pathreplacing,positioning}

\begin{figure}[t]
\centering
\resizebox{0.70\columnwidth}{!}{%
\begin{tikzpicture}[
    font=\scriptsize,
    box/.style={
        draw=gray!45,
        fill=gray!7,
        line width=0.7pt,
        minimum height=1.1cm,
        align=center
    },
    ptrbox/.style={
        draw=red!55,
        fill=red!5,
        line width=0.7pt,
        minimum height=1.1cm,
        align=center
    },
    pointer/.style={
        ->,
        very thick,
        red!55
    }
]

% Top Memory Blocks
\node[ptrbox, minimum width=1.6cm] (upper) {Upper\\Bound};
\node[box, minimum width=1.6cm, right=0pt of upper] (aux) {Aux\\Word};
\node[box, minimum width=6cm, right=0pt of aux] (payload) {Object Payload};

% Bottom Memory Blocks
% Positioned relative to the boundary of Payload for a clean parallel arrow effect
\node[ptrbox, minimum width=1.6cm, below=1.1cm of payload.south west, xshift=1cm, anchor=north west] (lower) {Lower\\Bound};
\node[box, minimum width=1.6cm, right=0pt of lower] (intval) {Pointer};

% Byte widths
\foreach \block in {upper,aux,lower,intval} {
    \draw[
        decorate,
        decoration={brace,mirror,amplitude=4pt}
    ]
        ([yshift=-2pt]\block.south west) --
        ([yshift=-2pt]\block.south east)
        node[midway, below=7pt] {8 bytes};
}

% The two-word capability stored with the object
\draw[
    decorate,
    decoration={brace,amplitude=5pt}
]
    ([yshift=2pt]upper.north west) --
    ([yshift=2pt]aux.north east)
    node[midway, above=8pt] {\InvisiCap{}};

% Labels and Annotations
\node[left=0.2cm of lower, font=\scriptsize] {Fil-C pointer:};

% Arrows
% Starting slightly above the center of the text blocks
\draw[pointer] ([yshift=0.2cm]lower.center) -- (payload.south west);

% Since the intval box is exactly 1.6cm to the right of the lower box,
% the arrow destination is shifted by exactly 1.6cm to keep them perfectly parallel.
\draw[dotted,pointer] ([yshift=0.2cm]intval.center) -- ([xshift=2.9cm]payload.south west);

% The upper-bound pointer targets the far end of the object.  The path
% leaves the box on the left, turns at (upper-route) and then sweeps
% above the InvisiCap label before descending onto the right-hand
% boundary of the payload.  Both control points next to (upper-route)
% are pure horizontal shifts, so the two Bezier segments share the same
% tangent there and meet without a kink; the final control point sits
% directly above the end point, so the arrow head comes down cleanly
% onto the boundary instead of overshooting it.
\coordinate (upper-route) at
    ([xshift=-0.2cm,yshift=0.8cm]upper.north west);
\draw[pointer]
    ([xshift=-0.5cm,yshift=0.2cm]upper.center)
    .. controls
        ([xshift=-0.25cm]upper.west) and
        ([xshift=-0.35cm]upper-route)
    .. (upper-route)
    .. controls
        ([xshift=2.9cm]upper-route) and
        ([yshift=0.9cm]payload.north east)
    .. (payload.north east);

\end{tikzpicture}%
}

\caption{Visualisation of a \FilC{} pointer and capability layout.}\label{fig:invisiCaps}

\end{figure}


==> figures/pipeline.tex <==
\begin{figure}[t]
\centering
\resizebox{0.62\columnwidth}{!}{%
\begin{tikzpicture}[font=\scriptsize, >=stealth,
   lane/.style={font=\scriptsize\itshape, text=black!75},
   note/.style={font=\tiny, text=black!55}]

  %% Shared start --- victim (\FilC{}) process
  \node[vicbox, text width=7.7cm, minimum height=0.60cm] (start) at (0,4.55)
       {\FilC{} victim allocates the object. Its \InvisiCap{} upper-bound word
      sits in ordinary DRAM};

  %% Lane titles
  \node[lane] at (-2.15,3.98) {Deterministic path};
  %\node[note] at (-2.15,3.70) {isolates the consequence};
  \node[lane] at ( 2.15,3.98) {Physical end-to-end path};
  \node[note] at ( 2.15,3.50) {proves delivery};

  %% Deterministic path --- one out-of-band write (attacker, native)
  \node[attbox, text width=3.15cm, minimum height=0.85cm] (det) at (-2.15,2.45)
     {Single out-of-band 1-bit write\\(\texttt{/proc/\textit{pid}/mem})};

  %% Physical end-to-end path --- Phases 1--3 (attacker, native)
  \node[attbox, text width=3.15cm] (p1) at (2.15,3.48) {Phase 1: DRAM templating};
  \node[attbox, text width=3.15cm] (p2) at (2.15,2.68) {Phase 2: Grooming};
  \node[attbox, text width=3.15cm] (p3) at (2.15,1.87) {Phase 3: Hammering};
  \draw[arr,-](p1)--(p2); \draw[arr,-](p2)--(p3);

  %% \FilC{} enforcement boundary: corruption crosses it out-of-band
  \draw[dashed,black!45] (-4.05,1.18) -- (4.05,1.18);
  \node[note] at (0,1.33) {\FilC{} enforcement boundary. Corruption happens out-of-band};

  %% Shared consequence --- Phase 4, victim (\FilC{}) process
  \node[vicbox, text width=7.7cm, minimum height=0.95cm] (cons) at (0,0.45)
     {\textbf{Phase 4 Exploitation (shared).}  The \FilC{} runtime treats the
      corrupted \texttt{upper} as authoritative and \emph{silently} permits the
      out-of-bounds access, without raising a panic, signal, or machine check};

  %% Start splits into the two paths
  \draw[arr](start.south-|det.north) -- (det.north);
  \draw[arr](start.south-|p1.north)  -- (p1.north);
  %% Each path lands the same corrupted capability, crossing the boundary
  \draw[darr,red!55](det.south) -- (det.south|-cons.north);
  \draw[darr,red!55](p3.south)  -- (p3.south|-cons.north);

\end{tikzpicture}%
}
\caption{The two experimental paths.  Blue boxes run inside the \FilC{} victim
process. Red boxes run in the attacker's native (non-\FilC{}) process.  Both
paths share the same start (a live \InvisiCap{} in DRAM) and the same
consequence (Phase~4: the runtime silently honours the corrupted bound). They
differ only in \emph{delivery}.  The \emph{deterministic path} lands the flip
with a single out-of-band write to isolate the metadata-corruption consequence.
The \emph{physical end-to-end path} lands it by real Rowhammer through
templating, grooming, and hammering (Phases~1--3).  Neither delivery is
mediated by a \FilC{} check, which is why the corruption is invisible to the
runtime.}
\label{fig:pipeline}
\end{figure}

